To Be or Not To Be a Verbal Multiword Expression: A Quest for Discriminating Features

Automatic identification of mutiword expressions (MWEs) is a pre-requisite for semantically-oriented downstream applications. This task is challenging because MWEs, especially verbal ones (VMWEs), exhibit surface variability. However, this variability is usually more restricted than in regular (non-VMWE) constructions, which leads to various variability profiles. We use this fact to determine the optimal set of features which could be used in a supervised classification setting to solve a subproblem of VMWE identification: the identification of occurrences of previously seen VMWEs. Surprisingly, a simple custom frequency-based feature selection method proves more efficient than other standard methods such as Chi-squared test, information gain or decision trees. An SVM classifier using the optimal set of only 6 features outperforms the best systems from a recent shared task on the French seen data.

==> mwe-examples-commands.tex <==
%%%%%%%%%%%
%% in-line examples for languages in Latin script
%%%%%%%%%%
\newcommand{\lex}[1]{\textbf{#1}}  %Lexicalized component
\newcommand{\litlex}[1]{\uwave{#1}}  %Literal reading of a lexicalized component
\newcommand{\coinlex}[1]{\dashuline{#1}}  %Coincindental co-occurrence of lexicalized components

\newcommand{\ile}[1]{\textsl{#1}} %In-line example  
\newcommand{\lit}[1]{`#1'} %Literal translation
\newcommand{\idio}[1]{`#1'}  %Idiomatic translation
\newcommand{\exlit}[2]{\ile{#1} \lit{#2}} %Example with a literal translation
\newcommand{\exidio}[2]{\ile{#1} \idio{#2}} %Example with an idiomatic translation
\newcommand{\litidio}[2]{\lit{#1}$ \Rightarrow $\idio{#2}} %Literal and idiomatic translation
\newcommand{\exlitidio}[3]{\ile{#1} \lit{#2}$ \Rightarrow $\idio{#3}} %Example with a literal and a and idiomatic translation



%%%%%%%%%%%
%% in-line examples for languages in non-Latin script
%%%%%%%%%%
%\newcommand{\nlile}[1]{#1} %In-line example  
\newcommand{\nlile}[1]{{#1}} %In-line example  
\newcommand{\nltli}[1]{#1} %Transliterated in-line example  

\newcommand{\nlextlilit}[3]{\nlile{#1}~(\nltli{#2})~\lit{#3}} %Example with a transliteration and a literal translation
\newcommand{\nlexlit}[2]{\nlile{#1}~\lit{#2}} %Example without a transliteration and with a literal translation
\newcommand{\nltlilit}[2]{\nltli{#1}~\lit{#2}} %A transliteration and a literal translation

\newcommand{\nlextliidio}[3]{\nlile{#1}~(\nltli{#2})~\idio{#3}} %Example with a transliteration and an idiomatic translation
\newcommand{\nltliidio}[2]{\nltli{#1}~\idio{#2}} %Example with an idiomatic translation
 
\newcommand{\nltlilitidio}[3]{\nltli{#1}~\lit{#2}$\Rightarrow$\idio{#3}} %Transliteration with a literal and an idiomatic translation
\newcommand{\nlextlilitidio}[4]{\nlile{#1}~(\nltli{#2})~\lit{#3}$\Rightarrow$\idio{#4}} %Example with a transliteration, a literal and an idiomatic translation
%%%%%%%%%%%

